Investigating the Role of Situational Disruptors in Engagement with Digital Mental Health Tools

Challenges in engagement with digital mental health (DMH) tools are commonly addressed through technical enhancements and algorithmic interventions. This paper shifts the focus towards the role of users' broader social context as a significant factor in engagement. Through an eight-week text messaging program aimed at enhancing psychological wellbeing, we recruited 20 participants to help us identify situational engagement disruptors (SEDs), including personal responsibilities, professional obligations, and unexpected health issues. In follow-up design workshops with 25 participants, we explored potential solutions that address such SEDs: prioritizing self-care through structured goal-setting, alternative framings for disengagement, and utilization of external resources. Our findings challenge conventional perspectives on engagement and offer actionable design implications for future DMH tools.

==> Draft/discussion.tex <==
\section{Discussion}

%Holistically viewing users' life

%\subsection{Key Insights}

\subsection{RQ1: Influence of SEDs in Dictating Engagement with DMH Tools}

%\todo{connect with engagement}

Our study offers nuanced insights into the HCI discussion around DMH tools, underscoring the intricate manner in which an individual's social context impacts their engagement with DMH tools. Central to our observations was the pervasive sense of being overwhelmed by various SEDs, including academic challenges, workplace expectations, familial duties, and unanticipated life events like health setbacks or relocations. While the specific circumstances and disruptors varied among individuals, there were commonalities across their experiences related to the feeling of overwhelm. This state often resulted in difficulty planning and prioritizing beyond immediate needs, along with increased distress about their broader situation. Such feelings led to failure to routine usage of the tool, even when participants expressed a genuine affinity for the platform and saw its potential benefits. Therefore, work that focuses on tweaking content, tailoring algorithms, or otherwise making superficial adjustments to a tool is unlikely to succeed in achieving engagement for populations facing mental health challenges, especially when considered over weeks or months.


%Although individuals' circumstances and specific disruptors varied widely, there were commonalities across their experiences as relating to the feeling of overwhelm, which included a loss of ability to plan and prioritize beyond meeting their most pressing obligations, as well as distress about their situation. Naturally, this typically resulted in failure to routinely use of a mental health tool, about which many participants felt some regret. These experiences of disruption occurred despite the users' best intentions. Indeed, participants reported generally liking the text messaging tool and the content it delivers, and thought it could be helpful to them. Thus, work that focuses on tweaking content or tailoring algorithms or otherwise making superficial adjustments to a tool is unlikely to succeed in achieving engagement for populations facing mental health challenges, especially when considered over weeks or months.

The intense sense of overwhelm stemming from academic and professional commitments may shed light on why participants in previous studies noted a preference for minimal to no support during work hours, even though there might be intermittent needs for respite and support \cite{bhattacharjee2023investigating, bhattacharjee2022design, howe2022design, wong2023mental}. Such pervasive stress can often relegate mental wellbeing initiatives to the sidelines, notably when the benefits of self-care practices remain intangible in the short term. In the face of a cascade of urgent responsibilities, participants reported frequently deferring self-care initiatives, finding themselves overshadowed by tasks with immediate deadlines and tangible rewards \cite{wong2023mental}. Compounding this challenge is the difficulty in maintaining a consistent healthy lifestyle. Factors such as shifts in dietary habits or disruptions in sleep patterns could further erode an individual's capacity to manage time efficiently \cite{gipson2019effects, karlgren2023sleep, lattie2020designing}. Such disturbances could adversely impact task performance and diminish the attention devoted to mental health practices.

Family obligations and financial concerns were also found to be important SEDs that can pervade every facet of an individual's life.  Prior research in the mental health domain has demonstrated the profound implications of several broad socio-economic factors, revealing their potential to exert adverse effects on mental wellbeing \cite{allen2014social, slavich2020social, tachtler2020supporting, guan2022financial, li2022suffered}. Our findings resonate with this narrative, emphasizing that these factors not only influence mental health but also play a pivotal role in determining the extent to which individuals engage with DMH tools. For instance, the demands of child-rearing can be a dominant source of stress, often leaving scarce opportunities for individuals to prioritize their self-care. Analogously, the weight of managing financial intricacies can exact a similar toll. These overarching social factors underscore the intertwined nature of life's responsibilities and their resultant influence on psychological wellbeing and engagement with DMH tools.


Our findings highlighted the importance of embracing a comprehensive understanding of users' lives when offering strategies to bolster psychological wellbeing \cite{pendse2022treatment, allen2014social, slavich2020social, murnane2018personal}. While self-management of psychological wellbeing could be perceived as an individual responsibility \cite{lorig2003self}, more recent studies have highlighted the limitations of such individualistic perspectives \cite{sallis2015ecological, murnane2018personal}, advocating for acknowledging the context in which an individual lives and is surrounded by.
In the context of our findings, this implies that DMH tools should factor in users' myriad responsibilities, life aspirations, daily routines, and social connections. A salient reason for disengagement, as indicated by our data, is users' struggle to align their engagement with DMH tools within the framework of their overarching goals and duties. In instances where such alignment falters, individuals often sideline their psychological wellbeing. This observation echoes earlier research advocating that mental health initiatives should resonate with the sociocultural milieu and life circumstances of individuals \cite{slavich2020social, slavich2023social, allen2014social, glanz2008health, tachtler2021unaccompanied, oguamanam2023intersectional, murnane2018personal}.


\subsection{RQ2: Designing DMH Tools to Account for the Social Contexts}

%Our findings underscored the importance of adopting a more holistic view of users' lives in the realm of DMH tool design, especially when it pertains to engagement. %Current tools like ours, often with a narrow focus on specific metrics or behaviors, may neglect the broader, interconnected aspects of users' daily lives, leading to decreased engagement and potential disconnection. Participants frequently voiced the sentiment that such tools, while well-intentioned, sometimes felt misaligned with their intricate realities, spanning personal, social, and professional spheres. This misalignment can result in tools feeling more burdensome than beneficial, prompting sporadic or short-lived engagement. To bolster sustained and meaningful user interaction, there is a pronounced need for tools that genuinely resonate with the multifaceted nature of users' experiences. Embracing a more holistic understanding of users' responsibilities, priorities, life goals, and surroundings, hence, will ensure that DMH tools are not just interacted with, but integrated into, the diverse tapestry of users' lives.

We recognize the complexity embedded in translating the understanding of broad SEDs into actionable design. Nevertheless, as elucidated below, our insights pave the way for design suggestions that can facilitate promising avenues for imminent DMH tools.


%This could necessitate users to input exhaustive details about their lives, or demand considerable computational capabilities, coupled with intensive tracking — all of which usher in privacy and ethical dilemmas \todo{cite}. 



%\subsection{Design Considerations}
\subsubsection{Streamlined Self-Care Through Structured Goal-Setting}


In line with previous studies \cite{bhattacharjee2022kind, brown2014health}, our findings underscore the difficulty users encounter when trying to weave self-care activities seamlessly into their daily lives. Conflicts arise when participants' perceived responsibilities, both familial and professional, interfere with the timing and perceived significance of these activities. Feedback from participants illuminates a pressing need: for tools that offer a clearer, more structured overview of their lives, assisting them in prioritizing their myriad responsibilities.

To effectively structure and compartmentalize these responsibilities, insights can be drawn from literature on collaborative goal-setting \cite{agapie2022longitudinal, lee2021sticky, hsueh2020exploring}. A plausible approach to simplifying complex objectives may be the use of guided conversations \cite{o2018suddenly, bowman2022pervasive}, designed to instruct users on breaking down broad objectives into distinct, actionable steps with rationales. Recognizing that these guided interactions might require thoughtful engagement, participants in our study suggested that such interventions be reserved for users' \textit{idle times} \cite{poole2013hci}. These idle times could include moments when individuals are engaged in low-attention activities, such as checking messages or browsing social networking platforms. Once a plan has been crafted, DMH tools could then offer occasional reminders, helping users to stay on track with the incremental steps needed to achieve their overall goals, thus facilitating a more manageable approach to balancing their myriad responsibilities.


Additionally, the challenge of recognizing the benefits of wellbeing activities over immediate academic or professional tasks can be addressed by implementing strategies that align with individuals' personalized goals and visually representing their progress. DMH tools could enable users to set personalized psychological wellbeing goals that correspond with their broader life objectives, highlighting the real-world implications of their self-care practices \cite{jennings2018personalized, lindhiem2016meta, agapie2022longitudinal}. Additionally, incorporating visual analytics tools as suggested in health and well-being visualization studies \cite{baumer2014reviewing, kocielnik2018reflection} could provide users with graphical representations of their wellbeing improvements, linking them to enhanced performance in other life areas. Further reinforcement can come from integrating educational modules that elucidate the scientific connections between wellbeing practices and work performance and overall life improvement \cite{howe2022design}. Through these combined approaches, users may be able to prioritize self-care amidst their manifold responsibilities.


%However, merely providing guided interactions may not be adequate, particularly when confronting multifaceted challenges and users are uncertain where to begin. Participants of our study indicated that there could be times they were not aware of existing resources or may not remember them. In such case,
%a supplementary approach could include sharing narratives of individuals navigating similar challenges or offering access to relevant community resources that can offer additional insight and guidance \cite{bhattacharjee2022kind, thaker2022exploring, baumel2018digital}.

%\todo{Should I add LLMs?}

%\todo{user may not know the importance, may need to be reminded}











%We also observed that participants indicated a need for scheduling such activities that would not clash with those responsibilities . 


\subsubsection{Designing for Flexible Engagement}

Our participants expressed a desire for greater flexibility when interacting with DMH tools. This need for adaptability spanned from a reimagined understanding of disengagement to diverse modes of interaction.

The core intent of DMH tools is to foster wellbeing, yet the overwhelming emphasis on sustained engagement can inadvertently defeat this purpose. Our research underscores that a relentless push for streaks and frequent notifications can introduce unnecessary stress. The daunting challenge of maintaining long streaks can discourage users from taking even small, incremental steps. A missed day of engagement might amplify feelings of setback. These observations resonate with prior studies that caution against over-gamifying engagement (e.g., focus on maintaining a streak, reaching a certain number of step counts) \cite{etkin2016hidden, bekk2022all, liu2017toward, jia2016personality, hamari2014does}. A more balanced approach that may allow users to derive value even from passive interactions or occasional breaks could be explored in this context. Rather than highlighting missed engagements, DMH tools should try to cultivate a foundational connection, nudging users gently during low engagement periods \cite{bhattacharjee2023integrating}.

This flexibility extends to the mode of interaction with DMH tools, as relying solely on a single mode, such as text messages, may not be suitable for all circumstances and may miss opportunities that might be captured through alternative means of communication. For instance, some individuals may find comfort in verbal communication when reflecting on stressful situations \cite{murray1994emotional, stigall2022towards}. Additionally, allowing users to respond via voice might provide an accessible option when their hands are occupied, such as when driving. People may also lack the concentration required to read lengthy texts when focused on other tasks \cite{bhattacharjee2022kind}, but images or animations could convey essential information in a more engaging manner \cite{bryant2003imaginal, howe2022design}. By incorporating flexibility to engage through diverse modes of communication, DMH tools can enhance accessibility and responsiveness to individual needs.

%Engagement is often key to aiding users in managing their wellbeing. However, many DMH tools appear overly preoccupied with sustaining user engagement. They frequently inundate users with notifications and emphasize maintaining streaks. While such features can be helpful in keeping users aligned with DMH tools, our study highlighted potential drawbacks. For some participants, the pursuit of maintaining streaks could inadvertently morph into a stressor. These streaks, perceived as lofty or unattainable, sometimes deter users from even initiating small, progressive steps. Conversely, an occasional lapse in engagement could leave users with the disheartening feeling of starting from scratch, undermining the very purpose of the tool. These findings extend the prior literature on quantifying and gamifying engagement \cite{etkin2016hidden, bekk2022all, liu2017toward, jia2016personality, hamari2014does}, by highlighting the potential negative impacts of streaks and rewards. As our participants reminded us, the goal of the DMH tools should instead be allowing users to manage their wellbeing, which might sometimes be possible through passive engagement by briefly skimming messages, or even allowing for occasional disengagement. In periods of low or no engagement, users should not be reminded about their failure to engage, rather they can be requested to have a baseline connection with DMH tools \cite{bhattacharjee2023integrating}.
%Thus, an overemphasis on maintaining unbroken streaks might sometimes be counterproductive.

\subsubsection{Multi-Level Interventions for Psychological Wellbeing Support}


Our findings emphasize the necessity for multi-level interventions that extend across various dimensions of life, including educational and workplace technologies, along with broader societal factors \cite{sallis2015ecological, scholmerich2016translating, bauer2022community, murnane2018personal}. In the educational and professional spheres, there exist  significant opportunities for organizations to weave mental health support into their existing technological infrastructure. Such integration acknowledges that mental wellbeing is not isolated from other facets of life but is intimately linked with work and study environments. Policy-level changes, as suggested by \citet{murnane2018personal}, could profoundly influence psychological well-being, either enhancing or deteriorating mental health support within organizations.

Building on the work of \citet{howe2022design}, interventions can be delivered at opportune moments identified through email interactions, digital calendar usage, or physiological data monitored in office settings. The inclusion of close relations and peers in an individual's mental wellbeing initiatives can add another layer of support \cite{bhattacharjee2022kind, burgess2019think}. Participants in our study pointed out that intense periods of stress and overwhelm could be mitigated collectively with colleagues and peers, who support one another. DMH tools can further facilitate these interactions by enabling group support and shared narratives. This communal approach can not only validate emotions but foster a sense of belonging, encouraging individuals to face their struggles with a sense of solidarity and shared experience. 

Regarding other SEDs, such as challenges in carrying out family obligations and managing financial support, targeted interventions could be strategically implemented. For example, access to programs providing family counseling and parental education can help individuals navigate the complexities of familial responsibilities, thereby reducing associated stress \cite{chi2015systematic, smout2023enabling}. Financial literacy workshops and access to personal finance management tools can empower individuals to take control of their financial situations, mitigating anxiety and potential mental health deterioration \cite{boyd2016earned, mehra2018prayana}. Community-based partnerships with local banks and financial institutions might facilitate these workshops, providing a practical approach to managing financial intricacies \cite{dillahunt2022village, moulder2014hci}. Moreover, support for childcare, eldercare, or other family-related needs could be organized and distributed through community support groups, relieving some of the burdens on those juggling family and work \cite{gisore2012community, butler2012relationship, compton2015social, smout2023enabling}.

\todo{Should I add LLMs}


%tangibility
%quantifiability
%structure

%addressing overwhelm -- address life problems and goal setting

%community support -- other models and cscw papers



%\subsection{Designing Multi-Level Interventions}




%\subsection{Allowing People to See tangible Benefits}


%\subsection{Family, community}

%Social translucence 
%https://dl.acm.org/doi/fullHtml/10.1145/2775388 



Sign-up Survey



%audio-video what people are used to do


%personal holistic
%personalized
%individual personalization
%maybe subgroup

\todo{social contexts become disruptions -- check otter}

==> Draft/related.tex <==
\section{Related Work}

In our overview of related work, we first outline the diverse social factors that negatively impact psychological wellbeing.
We then describe how DMH tools, more specifically text messaging services, have been used to promote behavior change and psychological wellbeing.
We follow this overview with a discussion on the challenges that designers and users face in sustaining engagement with DMH tools.


\subsection{Frameworks on the Social Determinants of Mental Health}
The impact of social contexts on mental health has garnered significant attention in the fields of HCI and psychology \cite{alegria2018social, allen2014social, bhattacharjee2021understanding, lewis2019cultural, slavich2023social, tachtler2021unaccompanied, lattie2020designing, bhattacharjee2023integrating, slavich2020social}. 
\todo{People have developed frameworks, we ground our findings in the following ones:}
%Another related theory with some overlap
%Social factors are important
    %social determinant by Allen
    %Other works have looked into social experiences -- social safety theory

% while they impact mental health, not sure how much they impact engagement with mental health tools

%Plenty of research works have suggested that one's social and economic backgrounds play key roles in shaping one's mental health and state of mind. 
%Social determinants refer to the conditions in which people ``are born, grow, live, work, and age'' \cite{marmot2011global}. The concept of social determinants has its inspiration from social gradients \cite{honorio2021social}, which suggests that people with higher social status have a higher life expectancy and fewer health risks compared to those with lower status. Differences in social determinants have been found to stem from an unequal distribution of resources, and hence, ways to reduce the differences should incorporate targeted social and economic measures \cite{marmot2008closing}
%\todo{difficulty in using one word}

\subsubsection{Social Safety Theory}
One notable framework that researchers have employed to methodically structure conversations around this topic is the Social Safety Theory by \citet{slavich2020social}. This framework highlights two contrasting forces on one's life circumstances: (1) socially safe environments characterized by aspects like acceptance, stability, predictability, and harmony; and (2) socially threatening situations marked by aspects like conflict, turbulence, and unpredictability. Social Safety Theory suggests that these two components impose an observable impact on one's mental wellbeing. 
As an example, the repercussions of performing poorly on an examination can permeate beyond the academic sphere. It can lead to negative social evaluations and critiques from peers or family members, subsequently impacting self-esteem and social status \cite{diamond2022rethinking, noronha2018study, bhattacharjee2021understanding}. Similarly, losing a job is often regarded as a negative economic event, but it can also trigger the loss of close social connections within the workplace and a decline in social standing amongst friends and family members \cite{diamond2022rethinking, katz2017self}.

%\subsubsection{Another Name}
A pivotal study by \citet{allen2014social} examined how individuals' living conditions, working conditions, socio-economic standing, and surrounding environment influence their mental health outcomes. Allen et al. employed a multi-level framework to investigate these social determinants, suggesting preventive measures for mental health disorders in the general populace. Their framework integrated a life-course perspective that encompassed various life stages (e.g., childhood, adulthood), community-level contexts (e.g., the natural and built environment, primary healthcare), and country-level contexts (e.g., social and political factors, cultural norms). The study's findings highlighted the detrimental effects on mental health outcomes stemming from adverse situations like unemployment, inadequate education, and instances of gender discrimination.

%Various 
\subsection{Social Contexts as Determinants of Mental Health}
Several studies have delved into the connection between social factors and mental health across different settings  \cite{brydsten2018health, lecerof2015does, han2015social, reibling2017depressed, li2022suffered, groot2022impact, de2017gender, frik2023model, oguamanam2023intersectional}. 
For instance, a study by \citet{katz2017self} found a correlation between lower income and symptoms of depression and suicidal thoughts among transgender individuals in the USA. Similarly, a study by \citet{guan2022financial} found that economic factors like the ownership of tangible possessions and subjective experiences of financial strain were strong predictors of depressive symptoms. Elsewhere, Danish researchers demonstrated that youths living independently in subpar housing conditions were particularly vulnerable to mental health challenges \cite{groot2022impact}. Meanwhile, a study conducted during the COVID-19 pandemic observed that female parents of young children were experiencing higher stress levels than other demographic groups~\cite{li2022suffered}. 
% Collectively, these investigations reveal that mental health conditions can be notably susceptible to various socioeconomic challenges.
% , such as financial strain, housing conditions, and familial responsibilities.


%Research conducted by \citet{guan2022financial} revealed that  tangible possessions, non-collateralized debt, and personal assessments of financial strain, are relatively strong and persistent predictors of depressive symptoms. A group of Danish researchers concluded that youths living alone in poor housing conditions were particularly prone to mental health concerns~\cite{groot2022impact}. Another study reported that female parents of young children endured higher stress levels during the COVID-19 pandemic compared to other demographic groups~\cite{li2022suffered}. 
%These studies, along with others,  indicate that mental health conditions can be particularly susceptible to challenges such as financial difficulties, housing conditions, and familial responsibilities.


The diverse ways in which social factors intersect with mental health are exemplified in the experiences of various demographic groups. Academic performance is often a primary stressor for university students, although other factors like high expectations from parents, economic pressures, and relationship problems can also exacerbate their mental health \cite{de2016relationship, bruffaerts2018mental, bhattacharjee2021understanding, lattie2020designing}. Meanwhile, the mental health of immigrant youths can be detrimentally impacted by concerns such as fears of deportation and anxiety over families left in their home countries \cite{tachtler2021unaccompanied, tachtler2020supporting, jakobsen2017impact}. Older adults often face unique challenges that can impact their mental health: social isolation, physical health issues, caregiving stress, and cognitive decline \cite{carod2017social, mccrone2008paying, huisman2013socioeconomic}.
These studies underscore the complex interplay between socioeconomic hardships and mental health, reinforcing the necessity for comprehensive approaches that consider these socioeconomic contexts when addressing mental health challenges.

%\citet{starkey2013financial} also observed similar results for African women and suggested that treatment strategies should be adapted based on one's level of financial distress. Indicators of poor financial conditions like food insecurity, 
%A British study \cite{pevalin2017impact} found that consistently living in poor housing conditions can worsen mental health of youth and adults. 

%\todo{some study on stress during end of semester, start of new jobs, etc}

%\todo{social safety schemas -- maybe}

%\todo{while they impact mental health, not sure how much they impact engagement with mental health tools}

%\todo{look into literature doc, look into Shirley's summary}

\subsection{Text Messaging as a DMH Tool for Promoting
Behavior Change and Psychological Wellbeing}
\todo{sentence that emphasizes that text messages are a type of DMH tool}
In recent years, text messaging services have shown considerable success in supporting behavior change across various physical and mental health challenges \cite{haug2013efficacy, haug2013pre, yun2013text, suffoletto2023effectiveness, shalaby2022text, figueroa2022daily, bhandari2022effectiveness, villanti2022tailored, gipson2019effects}. For instance, \citet{villanti2022tailored} conducted a randomized controlled trial and found that a tailored text message intervention for socioeconomically disadvantaged smokers led to greater smoking abstinence rates, reduced smoking frequency, and increased desire to cease smoking compared to online resources. A similar study by \citet{liao2018effectiveness} demonstrated that frequent text messages (3-5 messages per day) can contribute to lower cigarette consumption rates among adult smokers. 
%Moreover, \citet{suffoletto2023effectiveness} highlighted the benefits of text messaging interventions for non-treatment-seeking young adults with hazardous drinking habits. Their study showed that messages providing feedback on drinking plans, alcohol consumption, and drinking limit goals resulted in sustained reductions in binge drinking days. 
Regarding other forms of behavior change, \cite{gipson2019effects} developed an interaction aimed at improving sleep hygiene among college students. 
Additionally, \citet{glasner2022promising} developed an intervention aimed at improving medication adherence and reducing heavy drinking in adults with HIV and substance use disorders. 
Other areas where text messaging has shown promise include weight management \cite{siopis2015systematic, donaldson2014text}, promoting physical activity \cite{kim2013text, smith2020text, murnane2020designing}, and enhancing vaccine uptake \cite{buttenheim2022effects, mehta2022effect}, among many others.

There has also been a surge of text-messaging services aimed to promote psychological wellbeing~\cite{kretzschmar2019can, chikersal2020understanding, rathbone2017use, inkster2018empathy, morris2018towards, stowell2018designing, kornfield2022meeting, agyapong2020changes}. The breadth of the content they cover and the goals they seek to support are vast. Most text messaging services employ therapeutic techniques from clinical psychology — cognitive behavioral therapy (CBT) \cite{willson2019cognitive}, dialectical behavior therapy (DBT) \cite{linehan2014dbt}, acceptance and commitment therapy (ACT) \cite{hayes2004acceptance}, and motivational interviewing \cite{hettema2005motivational} — to deliver personalized content. Text messages can function as reminders, assisting individuals in setting aside time for leisure and physical exercise \cite{bhattacharjee2023investigating, figueroa2022daily}. They can also facilitate expressions of gratitude, nudging individuals to reflect on life's positive aspects \cite{bhattacharjee2022design}. Furthermore, text messages can convey narratives, offering insights into how peers have navigated and surmounted challenging life situations, thereby aiding individuals in applying psychological strategies in their own lives \cite{bhattacharjee2022kind}. These advancements have spurred researchers to explore the potential of AI-powered chatbots to simulate human conversations and foster self-reflection \cite{inkster2018empathy, kocielnik2018reflection, tielman2017should}. The momentum in this domain has further accelerated with the recent rise of large language models (LLMs) \cite{van2023global, kumar2022exploring}.

There have been numerous initiatives that harness text messaging services to assist individuals in navigating their wellbeing during particularly stressful events \cite{agyapong2020changes, levin2019outcomes, arps2018promoting, nobles2018identification, bhattacharjee2023investigating, agyapong2022text4hope, agyapong2022text4hope}. \citet{agyapong2022text4hope} implemented such a system during the COVID-19 pandemic, dispatching daily support messages that led to decreased self-reported anxiety and stress. \citet{levin2019outcomes} combined psychoeducational content and reminders to assist those with bipolar disorder and hypertension. Meanwhile, \citet{arps2018promoting} tackled adolescent depression by sending daily gratitude-focused texts.

Yet, there are several challenges pertaining to one's individual and social contexts that could prevent text messaging systems and other DMH tools from providing more benefits to users. We discuss these issues in the next subsection.


% Various text messaging services have been used to help people manage wellbeing during critical periods. For example, Agyapong et al.
% [1] deployed a text messaging service to help people manage their
% mental wellness during the COVID-19 pandemic. The service sent
% daily supportive messages to people along with requests to reflect
% on their stress, anxiety, and depression level. The authors found
% that their messages were able to significantly reduce self-reported
% anxiety scores among users. Levin et al . [68] delivered messages
% ranging from psychoeducational texts, reminders, and EMA queries
% to help people with bipolar disorder and hypertension manage
% their symptoms. Arps et al . [2] were able to reduce depressive
% symptoms among adolescents by sending them daily gratitude mes-
% sages. Lastly, researchers have explored the design of artificially
% intelligent chatbots that try to promote self-refection by engaging
% users in human-like conversations [50, 59, 123]




%In the past few years, text messaging services have  been quite successful in supporting behavior change for a range of physical and mental health challenges \cite{haug2013efficacy, haug2013pre, yun2013text, suffoletto2023effectiveness, shalaby2022text, figueroa2022daily, bhandari2022effectiveness, villanti2022tailored}. For example, 
%\citet{villanti2022tailored} reported through a randomized controlled trial that a tailored text message intervention for socio-economically disadvantaged young adult smokers could result in greater smoking abstinence rates,  reductions in smoking frequency, and increased desire to quit compared to online quit resources. Deployment of a similar service \cite{liao2018effectiveness} suggested that frequent delivery of messages (3--5 messages every day) can promote lower cigarette consumption rates among adult smokers. \citet{suffoletto2023effectiveness} noted the benefits of text messaging interventions in helping non-treatment-seeking young adults with hazardous drinking habits, showing that messages that provided feedback on drinking plans, alcohol consumption, and drinking limit goals resulted in long-lasting reductions in binge drinking days. \citet{glasner2022promising} developed an intervention aimed at enhancing medication adherence and reducing heavy drinking in adults with HIV and substance use disorders. Other promising avenues for text messaging applications include weight management \cite{siopis2015systematic, donaldson2014text}, physical activity promotion \cite{kim2013text, smith2020text, murnane2020designing}, vaccine uptake \cite{buttenheim2022effects, mehta2022effect}, among many others.




\subsection{Challenges of Sustaining Engagement with DMH Tools}

%Despite the well-documented benefits provided by digital mental health tools, they face lots of challenges in engaging users. The commonly cited reasons involve the delivery of generic content that people fail to see the benefits of or how they might apply in their life. To reach a broader population, interventions often try to address issues that might apply to a broad group of people, but in doing so they risk being perceived as insincere or surface-level. Additionally, the intervention contents may also have limited variety; ultimately, users end up engaging with repeated content in a short timeframe, making them possess a negative attitude toward the novelty aspect of the intervention.

While DMH tools offer an array of benefits, their practical utility is often limited by several substantial challenges that hinder user engagement. One of the most frequently cited issues lies in the delivery of generic content. In an effort to achieve widespread accessibility and help the maximum number of people, digital interventions often take a generalist approach \cite{rennick2016health} that addresses issues broadly applicable to a diverse population. However, such interventions run the risk of being perceived as insincere or superficial, making users feel that the information is too generic to be truly valuable or that it fails to consider the nuanced complexities of their individual experiences \cite{bhattacharjee2023investigating, slovak2023designing}. 
In turn, users are led to question the applicability of generic content to their unique circumstances or how to implement the suggestions from such content in their daily lives \cite{lederman2014moderated, bhattacharjee2022design}.
A further complication arises from the limited content variety within these digital tools \cite{bhattacharjee2022design}. Users often encounter repetitive content in DMH tools. This can reduce the intervention's perceived novelty and create a sense of monotony, negatively impacting engagement and leading to boredom \cite{brown2014mobile}. %The lack of variety can disengage users, potentially diminishing the tool's effectiveness and user satisfaction.
Furthermore, DMH tools face the challenge of competing with various ongoing and urgent demands for user attention \cite{muench2017more}. Even with personalized content, these tools run the risk of being ignored if they do not intervene at opportune moments \cite{bhattacharjee2022design}. 


%Several research studies have focused on identifying the ideal time window to deliver interventions~\cite{figueroa2022daily, hardeman2019systematic, gonul2019expandable, lin2006fish, rabbi2015automated, goldstein2017return, konrad2015finding, ghandeharioun2016kind}. Some studies have relied on users' digital calendars to determine when to send massages~\cite{howe2022design}. Meanwhile, other studies have relied on information about users' physical or mental state, including self-reported stress scores~\cite{paredes2014poptherapy}, physiological data (e.g., heart rate \cite{clarke2017mstress}) or activity level (e.g., walking, running, or being in a vehicle \cite{ismail2022design}). These works often utilize personalization algorithms, such as contextual multi-armed bandit algorithms \cite{figueroa2023ratings, li2010contextual}, to determine the timing and content of interventions that will have the highest likelihood of benefiting and engaging each user. By leveraging personalized algorithms and considering various contextual factors, DMH tools aim to optimize their interventions to be delivered when they are most likely to have an impact and capture the user's attention.

%\todo{review lit from https://www.jmir.org/2021/3/e24387/

%Literature has explored the impact of technology design on user engagement, but the profound role of social context has largely been unrecognized. Predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} anchor their analyses on factors such as perceived usefulness and ease of use. Social influence is included to a lesser extent, but only basic elements like peer influence or subjective norms. These models frequently overlook the nuanced interplay between users and their diverse social environments: familial ties, workplace rules and responsibilities, and broader societal interactions. Given the known significance of these dynamics in influencing mental health \cite{allen2014social, lattie2020designing, slavich2023social}, our work seeks to explore their role in determining the effectiveness and receptiveness of digital interventions.




Researchers have endeavored to address these barriers and enhance engagement with DMH tools through adjustments in tool design or by tailoring algorithms to ensure personalization in terms of content, timing, or delivery method \cite{doherty2012engagement, harding2015hci, poole2013hci, xu2013designing, howe2022design}. This view is also prominent in the design of influential technology adoption models. Models such as the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} have centered on factors like perceived usefulness and ease of use. Social influence has been included but to a lesser extent, with an emphasis on rudimentary elements such as peer influence and subjective norms.

However, there is a lack of comprehension about the dynamics of engagement in the context of an individual's life circumstances, which makes it challenging to determine whether the right approach to promote engagement requires only minor adjustments or calls for a more fundamental reassessment. At least in the context of DMH tools, prior research on various social contexts and their associations with psychological wellbeing  \cite{bhattacharjee2023investigating, alegria2018social, allen2014social, bhattacharjee2021understanding, lewis2019cultural, slavich2023social, tachtler2021unaccompanied, lattie2020designing, bhattacharjee2023integrating, slavich2020social} suggests that unexplored facets, particularly those tied to diverse social environments like familial relationships, workplace obligations, and broader societal interactions, may demand more profound alterations in how engagement with DMH tools is perceived. These experiences might be multifaceted and unpredictable, impacting a substantial subset of users suddenly and leading to disruptions or even halting tool use entirely. Therefore, it might be crucial to conceptualize tools that can assist users in overcoming challenges without disturbing tool functionality. This consideration may help maintain the user's relationship with the system for future use. %Moreover, tools may be crafted to navigate specific disruptors, signifying that they can be advantageous not merely in spite of these challenges but actually for addressing them.














%HCI and implementation science have tried to promote engagement of DMH tools and in general technology by making adjustments in the design of a tool or tailoring algorithms to ensure personaliztion in terms of content, timing, or delivery method. In the context of technology adoption, predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} have been built upon factors such as perceived usefulness and ease of use, with social influence included to a lesser extent, focusing on basic elements like peer influence or subjective norms. 


%There is a prevailing lack of understanding regarding the mechanics of engagement hampers our ability to ascertain whether the right approach involves only superficial modifications or calls for a more fundamental reassessment.
%At least in the context of DMH tools, prior works on various social contexts and their connections with psychological wellbeing indicate that there could be other aspects, particularly those related to diverse social environments: familial ties, workplace rules and responsibilities, and broader societal interactions, that have not been thoroughly explored and might require more profound changes to how we view engagement in the context of DMH tools. These experiences could be diverse and hard to predict. they affect a significant subset of users at a given moment, and stall or disrupt use of a tool in a dramatic way. It is important to think about designing tools that can help users "weather" challenges without disrupting tool use. This can keep the relationship to the system in place so they have ability to use it when they have ability in the future. Tools may also be designed so that can be helpful in navigating specific disruptors, i.e. they can be helpful *for* and not just *in spite of* disruptors.




%Research on engagement with DMH tools, as well as various other forms of technology, has largely concentrated on making minor adjustments or aligning the tool with the specific circumstances of users. Predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} anchor their analyses on factors such as perceived usefulness and ease of use, with social influence included to a lesser extent, focusing on basic elements like peer influence or subjective norms. Nevertheless, there could be other aspects, particularly those related to disruptions or challenging life situations, that have not been thoroughly explored and might require more profound changes to the content, delivery timing, and method. The prevailing lack of understanding regarding the mechanics of engagement hampers our ability to ascertain whether the right approach involves only superficial modifications or calls for a more fundamental reassessment.  This perspective emphasizes the need for a thorough examination of the complex interplay between tool use and life circumstances, to ensure a more resilient and adaptive design.




%Such dynamics, integral to a user's life, can profoundly shape priorities, receptiveness to digital interventions, and even the interpretation of content.



%Comparison With Other Models of Technology and Digital Health Intervention Engagement
%}

%However,  DMH tools have to compete with many ongoing and often urgent issues for getting user attention \cite{muench2017more}, and even with a variety of personalized contents, they face the risk of being ignored, if they do not intervene users at opportune moments \cite{bhattacharjee2022design}. Many research works have attempted to identify the ideal time window to deliver interventions \cite{figueroa2022daily, hardeman2019systematic, gonul2019expandable, lin2006fish, rabbi2015automated, goldstein2017return, konrad2015finding, ghandeharioun2016kind}; some have used sensors to anticipate their physical state (e.g., heart rate) \citet{clarke2017mstress} and activity level (e.g., walking, on vehicle) \cite{ismail2022design} and deliver interventions accordingly, some have relied on user-reported scores \cite{paredes2014poptherapy}, some others have prompted users in between meetings from digital calendars \cite{howe2022design}. This line of work relies on personalization algorithms (e.g.,  contextual multi-armed bandit algorithm \cite{figueroa2023ratings, li2010contextual}) to identify the timing and content of interventions that have the highest probability to benefit and receive engagement from a particular user.


%\todo{Social and Broader issues}
%However, a major limitation in much of the HCI literature is that disengagement with DMH tools is often viewed individualistically; technologies try to identify suitable times for intervening users or deliver contents that can address their state of mind or activity. But there are numerous external barriers that can cause users to not engage with DMH tools, many of which may not be within the control of the users. These barriers can contribute to user engagement in nuanced ways that cannot be captured by the collection of individual behavioral markers. 

%\todo{adaptive algos are yet to capture external factors}
%However, a significant limitation in much of the HCI literature is that disengagement with Digital Mental Health (DMH) tools is often viewed from an individualistic perspective, focusing primarily on individual factors without considering the broader social context in which individuals live. 
%Prior research suggests that an individual's mental health and state of mind are influenced by a range of social and environmental factors, including their financial status, career prospects, and familial responsibilities \todo{cite}. 
%These external factors may significantly impact an individual's engagement with DMH tools, but their influence is often underexplored in the literature. \todo{algorithms cannot capture them}
%Recognizing the importance of understanding how these external factors impact engagement with DMH tools, we aimed to investigate the interplay between these factors and users' engagement with DMH tools.

==> Old-CHI/related.tex <==
\section{Related Work}

In our overview of related work, we first outline the diverse social factors that negatively impact psychological wellbeing.
We then describe how DMH tools, more specifically text messaging services, have been used to promote behavior change and psychological wellbeing.
We follow this overview with a discussion on the challenges that designers and users face in sustaining engagement with DMH tools.

\subsection{Social Context and Individual Challenges as Determinants of Psychological Wellbeing}

Several frameworks have been developed in recent years to explain the role of social context and individual challenges as determinants of psychological wellbeing \cite{slavich2020social, slavich2023social, allen2014social, glanz2008health, tachtler2021unaccompanied, oguamanam2023intersectional, sallis2015ecological}. Among these, the Social Safety Theory by \citet{slavich2020social} provides insights into the dichotomy of (1) socially safe environments characterized by elements such as acceptance, stability, and harmony and (2) socially threatening situations marked by elements such as conflict, turbulence, and unpredictability. According to the theory, socially threatening situations can exert a considerable impact on one's psychological wellbeing. Examples of this can be found in everyday situations like performing poorly on an exam or losing a job. These events can extend beyond their immediate academic or economic effects, leading to negative social evaluations, a decline in self-esteem, and a shift in social status \cite{diamond2022rethinking, noronha2018study, bhattacharjee2021understanding, katz2017self}. Adding to this understanding, a study by \citet{allen2014social} delved into the complex interplay between living and working conditions, socio-economic standing, and the surrounding environment. Through a multi-level framework that encompassed various life stages and contextual factors, they illuminated the detrimental mental health consequences stemming from adverse situations such as unemployment, inadequate education, and instances of gender discrimination.


Many studies have delved into the connections between social factors and psychological wellbeing across diverse settings and demographic groups \cite{brydsten2018health, lecerof2015does, han2015social, reibling2017depressed, li2022suffered, groot2022impact, de2017gender, frik2023model, oguamanam2023intersectional, murnane2018personal}. For example, economic challenges have been found to significantly impact psychological wellbeing. A study by \citet{guan2022financial} discovered that tangible possessions and financial strain were strong predictors of depressive symptoms, while a study by \citet{katz2017self} found a correlation between lower income and symptoms of depression among transgender individuals in the USA. Among university students, academic performance, parental expectations, and economic stress have been identified as primary stressors \cite{de2016relationship, bruffaerts2018mental, lattie2020designing}. The psychological wellbeing of older adults has also been explored, with unique challenges including social isolation and physical health issues \cite{carod2017social, mccrone2008paying}. Additional studies have illuminated the diverse ways social factors can intersect with psychological wellbeing, such as immigrant youths fearing deportation \cite{tachtler2021unaccompanied, tachtler2020supporting} and parents experiencing stress during the COVID-19 pandemic \cite{li2022suffered}.

%\todo{multi-level interventions}
%https://dl.acm.org/doi/pdf/10.1145/3274396?casa_token=vo9GehKfd44AAAAA:6_PcS6e8RsNOVzEazag2mnfcPHoERYmW73sgsJBKide_EhIIVcpeGr63xzIhDlua4xGz1sshew4ER44

%Recognizing the influence of various social and economic challenges on mental health outcomes, researchers have advocated for multi-level interventions that holistically address mental health by considering an array of social and economic factors affecting individual lives \cite{aubry2016multiple, kerman2018effects, leung2015household, murnane2018personal, sallis2015ecological, li2010stage}. 

Recognizing the influence of various social and economic challenges on mental health outcomes, some studies developed targeted interventions that address the unique challenges faced by specific groups. These groups include but are not limited to low-income populations, minoritized populations, and those at risk of homelessness \cite{aubry2016multiple, kerman2018effects, leung2015household, murnane2018personal, sallis2015ecological, li2010stage, schueller2019use}. Interventions in this space are structured to account for the technological resources available to these targeted populations and the underlying issues contributing to their mental health conditions. 
For instance, targeted efforts to improve housing conditions have been shown to lessen the demand for inpatient psychiatric services among the homeless who suffer from mental disorders \cite{kerman2018effects}. %Additionally, initiatives promoting community involvement to build neighborhood trust and safety have yielded positive mental health outcomes \cite{butler2012relationship, compton2015social}. 
Other studies advocate for the consideration of temporal aspects like daily routines and life transitions when crafting interventions for psychological wellbeing \cite{doherty2010fieldwork, murnane2018personal, reddy2006temporality}. Implementation science literature \cite{graham2020implementation, urquhart2020defining, powell2015refined} complements these works by emphasizing the importance of social context and structures that can either facilitate or impede the effective use of mental health resources. Rather than concentrating solely on tool design, this field explores strategies for the successful deployment of existing tools in specific settings. Such strategies often include user and staff training as well as monitoring tool uptake \cite{powell2015refined, powell2012compilation}. Collectively, these works underscore the importance of a holistic approach that integrates mental wellbeing considerations into broader societal contexts. 



%Relatedly, the implementation science literature focuses on the real-world contexts and structures around tool use that can either support or undermine it. This work is less focused on how tools are designed, but rather the strategies for successfully deploying established tools in particular settings (e.g., providing training to users and organizational staff, monitoring uptake). These works collectively underscore the importance of a holistic approach, integrating mental well-being considerations into broader societal contexts.  
%Efforts in this avenue include developing initiatives to improve housing stability, which has been linked to decreased use of inpatient psychiatric hospitals among homeless people with mental illnesses \cite{kerman2018effects}, and enhancing neighborhood trust and safety through community participation, with beneficial impacts on mental health \cite{butler2012relationship, compton2015social}. Past work \cite{doherty2010fieldwork, murnane2018personal, reddy2006temporality} has also advocated for considering temporal layer that represents patterns and transitions throughout the course of the individual’s life and integrating wellbeing support with organizational entities.   


%Community-based interventions have sought to enhance neighborhood trust and safety and mitigate violence and crime, with beneficial impacts on mental health \cite{butler2012relationship, compton2015social}. Interventions  have also been identified as having a positive impact on mental wellbeing \cite{webber2017review, murnane2018personal}. \citet{murnane2018personal} 

%Urban planning programs focusing on access to green spaces have demonstrated potential in reducing depressive symptoms \cite{larson2016public, mceachan2016association}, and targeted programs to engage youth through social media and community organizations have positively influenced various behavioral health outcomes \cite{dunne2017review}. 


%\todo{interventions from this paper https://link.springer.com/article/10.1007/s11920-018-0969-9#Sec4}
%\todo{community level interventions from this paper https://link.springer.com/article/10.1007/s11920-018-0969-9#Sec4}


\subsection{Text Messaging as a DMH Platform for Promoting
Behavior Change and Psychological Wellbeing}
%\todo{sentence that emphasizes that text messages are a type of DMH tool}
Text messaging has emerged as a powerful DMH platform, providing an accessible and personalized means of supporting individuals in their health journeys. The broad reach of this medium extends across various demographic groups, making it particularly useful for populations that encounter obstacles in accessing more conventional digital platforms like apps and online programs \cite{muench2017more, bhattacharjee2022kind}.
In recent years, text messaging interventions have shown considerable success in supporting behavior change across various physical and mental health challenges \cite{haug2013efficacy, haug2013pre, yun2013text, suffoletto2023effectiveness, shalaby2022text, figueroa2022daily, bhandari2022effectiveness, villanti2022tailored, gipson2019effects}. For instance, \citet{villanti2022tailored} conducted a randomized controlled trial and found that a tailored text message intervention for socioeconomically disadvantaged smokers led to greater smoking abstinence rates, reduced smoking frequency, and increased desire to cease smoking compared to online resources. A similar study by \citet{liao2018effectiveness} demonstrated that frequent text messages (3-5 messages per day) could contribute to lower cigarette consumption rates among adult smokers. 
%Moreover, \citet{suffoletto2023effectiveness} highlighted the benefits of text messaging interventions for non-treatment-seeking young adults with hazardous drinking habits. Their study showed that messages providing feedback on drinking plans, alcohol consumption, and drinking limit goals resulted in sustained reductions in binge drinking days. 
Regarding other forms of behavior change, \citet{gipson2019effects} developed an intervention to improve sleep hygiene among college students, and \citet{glasner2022promising} developed an intervention to improve medication adherence and reduce heavy drinking in adults with HIV and substance use disorders. 
Other areas where text messaging has shown promise include weight management \cite{siopis2015systematic, donaldson2014text}, promoting physical activity \cite{kim2013text, smith2020text, murnane2020designing}, and enhancing vaccine uptake \cite{buttenheim2022effects, mehta2022effect}, among many others.

There has also been a surge of text-messaging services aimed at promoting psychological wellbeing~\cite{kretzschmar2019can, chikersal2020understanding, rathbone2017use, inkster2018empathy, morris2018towards, stowell2018designing, kornfield2022meeting, agyapong2020changes}. The breadth of the content they cover and the goals they seek to support are vast. Most text messaging services employ therapeutic techniques from clinical psychology — cognitive behavioral therapy \cite{willson2019cognitive}, dialectical behavior therapy \cite{linehan2014dbt}, acceptance and commitment therapy \cite{hayes2004acceptance}, and motivational interviewing \cite{hettema2005motivational} — to deliver support. Text messages can function as reminders, assisting individuals in setting aside time for leisure and physical exercise \cite{bhattacharjee2023investigating, figueroa2022daily}. They can also facilitate expressions of gratitude, nudging individuals to reflect on life's positive aspects \cite{bhattacharjee2022design}. Furthermore, text messages can share narratives that offer insights into how peers have navigated and surmounted challenging life situations, thereby aiding individuals in applying psychological strategies in their own lives \cite{bhattacharjee2022kind}. %These advancements have spurred researchers to explore the potential of AI-powered chatbots to simulate human conversations and foster self-reflection \cite{inkster2018empathy, kocielnik2018reflection, tielman2017should}. The momentum in this domain has further accelerated with the recent rise of large language models (LLMs) \cite{van2023global, kumar2022exploring}.

Several studies have leveraged the utility of text messaging as a medium to offer support for individuals grappling with various mental health challenges \cite{agyapong2020changes, levin2019outcomes, arps2018promoting, nobles2018identification, bhattacharjee2023investigating, agyapong2022text4hope}. \citet{agyapong2022text4hope} implemented such a system during the COVID-19 pandemic, dispatching daily support messages that led to decreased self-reported anxiety and stress. \citet{levin2019outcomes} combined psychoeducational content and reminders to assist those with bipolar disorder and hypertension. Meanwhile, \citet{arps2018promoting} tackled adolescent depression by sending daily texts centered around gratitude. Yet, there are several challenges pertaining to one's individual and social context that could prevent text messaging systems and other DMH tools from providing more benefits to users. We discuss these issues in the next subsection.


% Various text messaging services have been used to help people manage wellbeing during critical periods. For example, Agyapong et al.
% [1] deployed a text messaging service to help people manage their
% mental wellness during the COVID-19 pandemic. The service sent
% daily supportive messages to people along with requests to reflect
% on their stress, anxiety, and depression level. The authors found
% that their messages were able to significantly reduce self-reported
% anxiety scores among users. Levin et al . [68] delivered messages
% ranging from psychoeducational texts, reminders, and EMA queries
% to help people with bipolar disorder and hypertension manage
% their symptoms. Arps et al . [2] were able to reduce depressive
% symptoms among adolescents by sending them daily gratitude mes-
% sages. Lastly, researchers have explored the design of artificially
% intelligent chatbots that try to promote self-refection by engaging
% users in human-like conversations [50, 59, 123]




%In the past few years, text messaging services have  been quite successful in supporting behavior change for a range of physical and mental health challenges \cite{haug2013efficacy, haug2013pre, yun2013text, suffoletto2023effectiveness, shalaby2022text, figueroa2022daily, bhandari2022effectiveness, villanti2022tailored}. For example, 
%\citet{villanti2022tailored} reported through a randomized controlled trial that a tailored text message intervention for socio-economically disadvantaged young adult smokers could result in greater smoking abstinence rates,  reductions in smoking frequency, and increased desire to quit compared to online quit resources. Deployment of a similar service \cite{liao2018effectiveness} suggested that frequent delivery of messages (3--5 messages every day) can promote lower cigarette consumption rates among adult smokers. \citet{suffoletto2023effectiveness} noted the benefits of text messaging interventions in helping non-treatment-seeking young adults with hazardous drinking habits, showing that messages that provided feedback on drinking plans, alcohol consumption, and drinking limit goals resulted in long-lasting reductions in binge drinking days. \citet{glasner2022promising} developed an intervention aimed at enhancing medication adherence and reducing heavy drinking in adults with HIV and substance use disorders. Other promising avenues for text messaging applications include weight management \cite{siopis2015systematic, donaldson2014text}, physical activity promotion \cite{kim2013text, smith2020text, murnane2020designing}, vaccine uptake \cite{buttenheim2022effects, mehta2022effect}, among many others.




\subsection{Challenges of Sustaining Engagement with DMH Tools}

%Despite the well-documented benefits provided by digital mental health tools, they face lots of challenges in engaging users. The commonly cited reasons involve the delivery of generic content that people fail to see the benefits of or how they might apply in their life. To reach a broader population, interventions often try to address issues that might apply to a broad group of people, but in doing so they risk being perceived as insincere or surface-level. Additionally, the intervention contents may also have limited variety; ultimately, users end up engaging with repeated content in a short timeframe, making them possess a negative attitude toward the novelty aspect of the intervention.

%While DMH tools offer an array of benefits, their practical utility is often limited by several substantial challenges that hinder user engagement. Researchers have quantified engagement in numerous ways, such as days of sustained use, user responsiveness, and daily sessions of use \todo{cite}. To study engagement, studies have examined who is likely to initiate and sustain engagement with DMH tools, finding that individuals who are more highly motivated for behavior change tend to sustain use. Studies have examined who is likely to initiate and sustain engagement with DMH tools, finding that individuals who are more highly motivated for behavior change tend to sustain use...Studies also show that engagement tends to be low. For example, users engage with downloaded mental health apps an average of... This suggests that many individuals may not have exposure to tools sufficient to learn and apply new skills. Indeed, research shows that greater engagement also tends to predict greater levels of benefit from using a tool. 


Although there is no universal conceptualization of engagement for DMH tools \cite{zech2023integrative}, researchers have quantified engagement in several ways: days of sustained use, user responsiveness, frequency of daily sessions, etc. \cite{lipschitz2023engagement, wang2023metrics}. Regardless of the metric, studies often report low engagement rates with DMH tools \cite{baumel2019objective, lipschitz2023engagement}. \citet{baumel2019objective} reported that individuals with a mental health app installed exhibit a median daily open rate of 4.0\%, and the 15-day median retention rate stands at  3.9\%. These statistics suggest that users might access mental health apps sporadically, and engagement beyond the first 15 days is uncommon. This poses a challenge for DMH tools, as sustained engagement has been significantly related to improved mental health outcomes \cite{gan2021effect}.


%While DMH tools offer a range of benefits, their effectiveness is often undermined by challenges that limit user engagement. Researchers have defined engagement in multiple ways, such as days of sustained use, user responsiveness, and frequency of daily sessions \cite{lipschitz2023engagement, wang2023metrics}. %Previous studies have indicated that individuals with higher motivation for behavioral change may be more likely to sustain engagement. Despite this, general engagement levels are often low, implying that many users do not interact with these tools enough to derive significant benefits \cite{gan2021effect}. Some works have focused on early identification of users who may face engagement challenges, aiming to provide them with additional support, such as coaching. However, our study aims to show a more nuanced perspective, showing whether motivated individuals can disengage due to disruptions stemming from social context. In that case, the measurement of initial engagement in the first days or weeks may not be an accurate predictor of long-term usage, as life circumstances can disrupt even initially committed users.

Prior work has identified some elements of DMH tools that can cause disengagement. A common issue is the use of generic and repetitive content \cite{bhattacharjee2022design, rennick2016health, brown2014mobile}. While aiming for a wide reach, DMH interventions risk seeming insincere as generalized material may not resonate with users' unique situations \cite{bhattacharjee2023investigating, slovak2023designing}. This lack of personal relevance, compounded by limited content variety, often leads to decreased engagement due to monotony and boredom \cite{brown2014mobile}.
%A common criticism lies in the delivery of generic content \cite{bhattacharjee2022design}. Aiming at broader reach, digital interventions often take a generalist approach \cite{rennick2016health} that addresses issues broadly applicable to a diverse population. However, such interventions risk appearing insincere, as users may find the content too generic and question its relevance to their unique situations or how to apply its suggestions in daily life. \cite{bhattacharjee2023investigating, slovak2023designing}. 
%A further complication arises from the limited content variety within these digital tools \cite{bhattacharjee2022design}. Users often encounter repetitive content in DMH tools, reducing perceived novelty and creating a sense of monotony that can negatively impact engagement and lead to boredom \cite{brown2014mobile}. %The lack of variety can disengage users, potentially diminishing the tool's effectiveness and user satisfaction.
Furthermore, DMH tools face the challenge of competing with various ongoing and urgent demands for user attention \cite{muench2017more}. Even with personalized content, these tools run the risk of being ignored if they do not intervene at opportune moments \cite{bhattacharjee2022design}. 

%Several research studies have focused on identifying the ideal time window to deliver interventions~\cite{figueroa2022daily, hardeman2019systematic, gonul2019expandable, lin2006fish, rabbi2015automated, goldstein2017return, konrad2015finding, ghandeharioun2016kind}. Some studies have relied on users' digital calendars to determine when to send massages~\cite{howe2022design}. Meanwhile, other studies have relied on information about users' physical or mental state, including self-reported stress scores~\cite{paredes2014poptherapy}, physiological data (e.g., heart rate \cite{clarke2017mstress}) or activity level (e.g., walking, running, or being in a vehicle \cite{ismail2022design}). These works often utilize personalization algorithms, such as contextual multi-armed bandit algorithms \cite{figueroa2023ratings, li2010contextual}, to determine the timing and content of interventions that will have the highest likelihood of benefiting and engaging each user. By leveraging personalized algorithms and considering various contextual factors, DMH tools aim to optimize their interventions to be delivered when they are most likely to have an impact and capture the user's attention.

%\todo{review lit from https://www.jmir.org/2021/3/e24387/

%Literature has explored the impact of technology design on user engagement, but the profound role of social context has largely been unrecognized. Predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} anchor their analyses on factors such as perceived usefulness and ease of use. Social influence is included to a lesser extent, but only basic elements like peer influence or subjective norms. These models frequently overlook the nuanced interplay between users and their diverse social environments: familial ties, workplace rules and responsibilities, and broader societal interactions. Given the known significance of these dynamics in influencing mental health \cite{allen2014social, lattie2020designing, slavich2023social}, our work seeks to explore their role in determining the effectiveness and receptiveness of digital interventions.

Researchers have endeavored to address these barriers and enhance engagement with DMH tools by refining features that inhibit engagement, making improvements in UI/UX, and tailoring algorithms to ensure content and delivery personalization \cite{doherty2012engagement, harding2015hci, poole2013hci, xu2013designing, howe2022design, lipschitz2023engagement}. This view toward engagement is also prominent in the design of influential technology adoption models, such as the Technology Acceptance Model (TAM) \cite{venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re}. %, or the Lived Informatics Model (LIM) \cite{epstein2015lived}. 
These models have centered on factors like perceived usefulness and ease of use. However, these factors have often been considered in isolation, neglecting the broader influences of one's surroundings. Social influence has been included but to a lesser extent, with an emphasis on elements such as peer influence and subjective norms \cite{marangunic2015technology}. Some initiatives have proactively identified individuals at risk of low engagement to implement adaptive interventions, such as providing specialized coaching or peer support to enhance their engagement \cite{arnold2019predicting, lipschitz2023engagement}. While we acknowledge that these efforts and models are important steps in improving engagement with DMH tools, there exists a lack of knowledge about the dynamics of engagement in the context of an individual's life circumstances. This gap makes it challenging to determine whether the right approach to promote engagement requires only minor adjustments in tool design or calls for a more fundamental reassessment.


%Prior research on various social and economic factors and their associations with psychological wellbeing suggests that unexplored disruptors, particularly those tied to diverse social environments like familial relationships, workplace obligations, and broader societal interactions, may demand more profound alterations in how engagement with DMH tools is perceived \cite{bhattacharjee2023investigating, alegria2018social, allen2014social, bhattacharjee2021understanding, lewis2019cultural, slavich2023social, tachtler2021unaccompanied, lattie2020designing, bhattacharjee2023integrating, slavich2020social}. 

%check the rewrite--rachel
Building on previous research that has thoroughly investigated the impact of diverse social and economic factors on mental health \cite{slavich2020social, mills2020prioritising, allen2014social}, we posit that fluctuations in social context could significantly impede the consistent and sustained engagement with DMH tools.
These disruptors of engagement are likely to be multifaceted, unpredictable, and possibly challenging to monitor \cite{bhattacharjee2022design, allen2014social, slavich2023social}. They can manifest broadly and suddenly, leading to unexpected disruptions or even causing individuals to halt engagement altogether. Traditional user studies spanning only a few days or weeks may fail to capture these disruptors \cite{bhattacharjee2022design}. Instead, the influence of these factors may only emerge over time as users with mental health concerns integrate DMH tools into their daily lives. 

In our first study, we aim to bridge this gap by extending our understanding of engagement with DMH tools. Through an eight-week-long study, we seek to identify these disruptors and provide a more comprehensive view of how these complex factors influence engagement. In our second study, we build on this knowledge by eliciting potential strategies for engaging end-users of DMH tools who are facing disruptors. 

%Therefore, it might be crucial to conceptualize tools that can assist users in overcoming challenges without disturbing tool functionality. This consideration may help maintain the user's relationship with the system for future use. Moreover, tools may be crafted to navigate specific disruptors, signifying that they can be advantageous not merely in spite of these challenges but actually for addressing them.


%These disruptors might be multifaceted,  unpredictable, and possibly difficult to monitor \cite{bhattacharjee2022design, allen2014social, slavich2023social}, impacting a substantial subset of users suddenly and leading to disruptions or even halting tool use entirely. Shorter user studies of a few days or a couple of weeks may not capture these SEDs \cite{bhattacharjee2022design}, rather they may emerge over time among users with mental health concerns as they engage a tool in daily life.
%\todo{review 2.3}










%HCI and implementation science have tried to promote engagement of DMH tools and in general technology by making adjustments in the design of a tool or tailoring algorithms to ensure personaliztion in terms of content, timing, or delivery method. In the context of technology adoption, predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} have been built upon factors such as perceived usefulness and ease of use, with social influence included to a lesser extent, focusing on basic elements like peer influence or subjective norms. 


%There is a prevailing lack of understanding regarding the mechanics of engagement hampers our ability to ascertain whether the right approach involves only superficial modifications or calls for a more fundamental reassessment.
%At least in the context of DMH tools, prior works on various social contexts and their connections with psychological wellbeing indicate that there could be other aspects, particularly those related to diverse social environments: familial ties, workplace rules and responsibilities, and broader societal interactions, that have not been thoroughly explored and might require more profound changes to how we view engagement in the context of DMH tools. These experiences could be diverse and hard to predict. they affect a significant subset of users at a given moment, and stall or disrupt use of a tool in a dramatic way. It is important to think about designing tools that can help users "weather" challenges without disrupting tool use. This can keep the relationship to the system in place so they have ability to use it when they have ability in the future. Tools may also be designed so that can be helpful in navigating specific disruptors, i.e. they can be helpful *for* and not just *in spite of* disruptors.




%Research on engagement with DMH tools, as well as various other forms of technology, has largely concentrated on making minor adjustments or aligning the tool with the specific circumstances of users. Predominant models like the Technology Acceptance Model (TAM) \cite{marangunic2015technology, venkatesh2008technology, davis1989perceived} and the Unified Theory of Acceptance and Use of Technology (UTAUT) \cite{venkatesh2003user, dwivedi2019re} anchor their analyses on factors such as perceived usefulness and ease of use, with social influence included to a lesser extent, focusing on basic elements like peer influence or subjective norms. Nevertheless, there could be other aspects, particularly those related to disruptions or challenging life situations, that have not been thoroughly explored and might require more profound changes to the content, delivery timing, and method. The prevailing lack of understanding regarding the mechanics of engagement hampers our ability to ascertain whether the right approach involves only superficial modifications or calls for a more fundamental reassessment.  This perspective emphasizes the need for a thorough examination of the complex interplay between tool use and life circumstances, to ensure a more resilient and adaptive design.




%Such dynamics, integral to a user's life, can profoundly shape priorities, receptiveness to digital interventions, and even the interpretation of content.



%Comparison With Other Models of Technology and Digital Health Intervention Engagement
%}

%However,  DMH tools have to compete with many ongoing and often urgent issues for getting user attention \cite{muench2017more}, and even with a variety of personalized contents, they face the risk of being ignored, if they do not intervene users at opportune moments \cite{bhattacharjee2022design}. Many research works have attempted to identify the ideal time window to deliver interventions \cite{figueroa2022daily, hardeman2019systematic, gonul2019expandable, lin2006fish, rabbi2015automated, goldstein2017return, konrad2015finding, ghandeharioun2016kind}; some have used sensors to anticipate their physical state (e.g., heart rate) \citet{clarke2017mstress} and activity level (e.g., walking, on vehicle) \cite{ismail2022design} and deliver interventions accordingly, some have relied on user-reported scores \cite{paredes2014poptherapy}, some others have prompted users in between meetings from digital calendars \cite{howe2022design}. This line of work relies on personalization algorithms (e.g.,  contextual multi-armed bandit algorithm \cite{figueroa2023ratings, li2010contextual}) to identify the timing and content of interventions that have the highest probability to benefit and receive engagement from a particular user.


%\todo{Social and Broader issues}
%However, a major limitation in much of the HCI literature is that disengagement with DMH tools is often viewed individualistically; technologies try to identify suitable times for intervening users or deliver contents that can address their state of mind or activity. But there are numerous external barriers that can cause users to not engage with DMH tools, many of which may not be within the control of the users. These barriers can contribute to user engagement in nuanced ways that cannot be captured by the collection of individual behavioral markers. 

%\todo{adaptive algos are yet to capture external factors}
%However, a significant limitation in much of the HCI literature is that disengagement with Digital Mental Health (DMH) tools is often viewed from an individualistic perspective, focusing primarily on individual factors without considering the broader social context in which individuals live. 
%Prior research suggests that an individual's mental health and state of mind are influenced by a range of social and environmental factors, including their financial status, career prospects, and familial responsibilities \todo{cite}. 
%These external factors may significantly impact an individual's engagement with DMH tools, but their influence is often underexplored in the literature. \todo{algorithms cannot capture them}
%Recognizing the importance of understanding how these external factors impact engagement with DMH tools, we aimed to investigate the interplay between these factors and users' engagement with DMH tools.
